Beyond Stars: MTTX Brings Developer Responsiveness to Dependency Decisions, from Dashboard to IDE to GitHub Actions

Modern software reuses open-source packages as dependencies, and developers often choose among candidate packages with cheap signals, such as GitHub stars and download counts. However, such signals are easy to fake, so developers need signals that represent "observed behavior," such as how quickly the developers of a package respond to new dependency releases and to security fixes. Prior work computed these responsiveness metrics, MTTU (Mean Time To Update) dependencies and MTTR (Mean Time To Remediate) vulnerable dependencies, but only with a research prototype for a fixed set of packages. Therefore, developers cannot easily benefit from them or integrate them into their workflow. We present MTTX, an open-source tool that computes MTTU and MTTR with accurate historical dependency resolution for any package and given time window, and brings them into different phases of developer workflow. MTTX resolves each version constraint of npm, PyPI, and Cargo packages as of a past date, with data from the native registries or deps.dev and vulnerability data from OSV. We validated MTTX with 328 automated tests, and for 90 packages from prior work, we manually verified its dependency resolution at each historical release point and its MTTU and MTTR computation. Developers can use MTTX in an interactive web dashboard, an IDE extension, and a GitHub Action, which are all available from the project homepage at https://imranur-rahman.github.io/dependency-update-metrics/. We envision that package registries (e.g., npm) and metadata aggregators and intelligence platforms (e.g., deps.dev) will display these values on the package page, alongside download counts and stars, to make them easier for developers to access. A demo video is at https://youtu.be/MZqjDnJ8bEQ.

==> figures/logos.tex <==
\newsavebox{\npmlogo}\newsavebox{\pypilogo}\newsavebox{\rustlogo}\newsavebox{\osvlogo}\newsavebox{\depsdevlogo}%
\sbox{\npmlogo}{\tikz\fill[brandnpm] svg {%
M -5.972 7.000 C -6.542 7.000 -7.000 6.542 -7.000 5.972 L -7.000 -5.972 C -7.000 -6.541
-6.542 -7.000 -5.972 -7.000 L 5.972 -7.000 C 6.542 -7.000 7.000 -6.541 7.000 -5.972 L
7.000 5.972 C 7.000 6.542 6.541 7.000 5.972 7.000 Z M -4.008 3.895 L 4.064 3.884 L 4.059
-4.187 L 2.038 -4.187 L 2.044 1.869 L 0.028 1.869 L 0.023 -4.183 L -4.017 -4.183 Z};}%
\sbox{\pypilogo}{\tikz\fill[brandpypi] svg {%
M 6.955 -0.922 L 6.955 -3.204 L 4.988 -3.920 L 4.942 -3.952 L 4.972 -3.974 L 6.985 -3.241
L 7.000 -3.220 L 7.000 -0.888 L 6.969 -0.867 L 6.955 -0.921 Z M 6.779 3.723 L 5.006 3.077
L 5.006 0.795 L 6.953 1.504 L 6.953 3.786 Z M 6.953 -0.850 L 6.953 1.433 L 5.007 0.724 L
5.007 -1.559 Z M 4.941 -1.581 L 4.941 0.700 L 3.016 0.000 L 3.016 -2.283 Z M 2.936 -4.664
L 2.936 -2.382 L 1.004 -3.086 L 1.004 -5.368 Z M 3.016 -2.367 L 3.016 -4.623 L 4.949
-3.919 L 4.949 -1.662 L 3.016 -2.366 Z M 4.237 -3.464 C 4.023 -3.543 3.850 -3.421 3.850
-3.194 C 3.850 -2.967 4.023 -2.719 4.237 -2.642 C 4.450 -2.564 4.623 -2.686 4.623 -2.913 C
4.623 -3.139 4.450 -3.387 4.237 -3.464 Z M 0.715 1.566 L 0.927 1.643 L -0.989 2.342 L
-2.927 1.636 L -2.868 1.614 L -1.010 0.937 Z M 4.962 0.779 L 4.962 3.062 L 3.016 2.354 L
3.016 0.071 Z M 2.950 0.048 L 2.950 2.330 L 1.024 1.629 L 1.024 -0.653 Z M 0.958 1.606 L
-0.988 0.898 L -0.988 -1.385 L 0.958 -0.676 Z M -2.971 -0.680 L -1.033 -1.385 L -1.033
0.898 L -2.971 1.603 Z M -0.968 2.407 L 0.946 1.711 L 0.946 3.968 L -0.968 4.664 Z M 4.962
5.416 L 3.028 4.712 L 3.028 2.430 L 4.962 3.134 Z M 2.887 4.723 L 1.006 5.407 L -0.901
4.713 L 0.980 4.029 Z M 1.963 4.313 L 1.016 3.968 L 1.016 1.712 L 2.950 2.416 L 2.950
4.672 L 1.963 4.313 Z M 1.735 2.693 C 1.521 2.614 1.349 2.736 1.349 2.963 C 1.349 3.191
1.521 3.438 1.735 3.515 C 1.948 3.593 2.122 3.472 2.122 3.244 C 2.122 3.017 1.948 2.770
1.735 2.693 Z M -1.033 -3.739 L -1.033 -1.456 L -2.971 -0.751 L -2.971 -3.033 Z M 0.979
-3.023 L 0.979 -0.740 L -0.988 -1.456 L -0.988 -3.739 Z M 1.024 -3.006 L 2.949 -2.307 L
2.949 -0.023 L 1.024 -0.723 Z M 0.979 -5.377 L -0.988 -6.092 L -0.988 -3.810 L -1.033
-3.810 L -1.033 -6.092 L -2.971 -5.387 L -2.971 -3.104 L -3.002 -3.071 L -3.016 -3.036 L
-4.962 -2.330 L -4.962 -0.027 L -4.943 -0.034 L -3.025 -0.732 L -3.016 -0.687 L -4.919
0.006 L -3.017 0.698 L -3.017 0.762 L -4.739 1.388 L -4.918 1.454 L -3.016 2.147 L -3.016
1.635 L -2.970 1.667 L -2.970 3.051 L -1.070 2.360 L -1.037 2.396 L -2.868 3.062 L -2.927
3.084 L -1.037 3.772 L -1.037 3.820 L -3.002 3.105 L -3.002 3.095 L -3.016 3.084 L -3.016
2.196 L -4.993 1.476 L -4.993 1.464 L -5.008 1.454 L -5.008 -0.883 L -6.985 -1.602 L
-6.985 -1.614 L -7.000 -1.624 L -7.000 -3.954 L -6.985 -3.976 L -5.002 -4.698 L -4.997
-4.694 L -4.993 -4.700 L -3.010 -5.422 L -3.005 -5.419 L -3.002 -5.424 L -1.019 -6.146 L
-1.010 -6.141 L -1.003 -6.147 L 1.009 -5.414 L 1.024 -5.392 L 0.979 -5.377 Z M -4.962
1.422 L -3.062 0.730 L -4.962 0.038 L -4.962 1.422 Z M -5.017 -4.643 L -6.955 -3.939 L
-6.955 -1.656 L -5.577 -2.158 L -5.017 -2.361 L -5.017 -4.644 Z M -5.008 -2.316 L -6.805
-1.662 L -6.911 -1.624 L -5.008 -0.932 L -5.008 -2.316 Z M -3.025 -5.367 L -4.962 -4.662 L
-4.962 -2.380 L -3.025 -3.085 L -3.025 -5.367 Z M 6.878 3.830 L 5.006 4.513 L 5.006 3.149
Z M 4.892 5.458 L 3.002 6.147 L 1.095 5.452 L 2.989 4.763 Z};}%
\sbox{\rustlogo}{\tikz\fill[brandrust] svg {%
M 6.904 0.173 L 6.316 0.537 C 6.311 0.594 6.306 0.651 6.299 0.708 L 6.804 1.179 C 6.855
1.227 6.877 1.298 6.864 1.366 C 6.850 1.434 6.802 1.491 6.737 1.516 L 6.092 1.757 C 6.076
1.813 6.059 1.869 6.041 1.924 L 6.443 2.483 C 6.485 2.540 6.493 2.614 6.466 2.679 C 6.440
2.744 6.381 2.790 6.312 2.801 L 5.631 2.911 C 5.605 2.963 5.578 3.014 5.549 3.064 L 5.835
3.692 C 5.865 3.756 5.858 3.830 5.819 3.888 C 5.780 3.946 5.714 3.980 5.644 3.978 L 4.953
3.954 C 4.918 3.999 4.881 4.043 4.844 4.086 L 5.003 4.759 C 5.019 4.827 4.998 4.898 4.949
4.948 C 4.899 4.998 4.827 5.018 4.759 5.002 L 4.087 4.843 C 4.043 4.880 3.998 4.916 3.954
4.952 L 3.978 5.643 C 3.981 5.714 3.948 5.781 3.889 5.820 C 3.831 5.859 3.756 5.865 3.692
5.835 L 3.064 5.548 C 3.014 5.576 2.963 5.604 2.911 5.630 L 2.800 6.311 C 2.789 6.380
2.742 6.438 2.678 6.465 C 2.613 6.492 2.540 6.483 2.483 6.443 L 1.923 6.040 C 1.868 6.058
1.812 6.075 1.756 6.090 L 1.515 6.736 C 1.490 6.801 1.433 6.849 1.365 6.863 C 1.296 6.876
1.226 6.854 1.178 6.803 L 0.707 6.298 C 0.650 6.304 0.593 6.310 0.536 6.314 L 0.172 6.902
C 0.135 6.961 0.070 6.998 0.000 6.998 C -0.070 6.998 -0.135 6.961 -0.172 6.902 L -0.536
6.314 C -0.593 6.309 -0.650 6.304 -0.707 6.298 L -1.178 6.803 C -1.226 6.854 -1.297 6.877
-1.366 6.864 C -1.434 6.850 -1.491 6.802 -1.515 6.736 L -1.757 6.090 C -1.813 6.074 -1.868
6.057 -1.923 6.040 L -2.483 6.443 C -2.540 6.483 -2.613 6.492 -2.678 6.465 C -2.742 6.438
-2.789 6.380 -2.800 6.311 L -2.911 5.630 C -2.963 5.604 -3.014 5.576 -3.064 5.548 L -3.692
5.835 C -3.756 5.864 -3.830 5.858 -3.889 5.819 C -3.947 5.780 -3.981 5.713 -3.978 5.643 L
-3.954 4.952 C -3.999 4.917 -4.043 4.880 -4.087 4.843 L -4.759 5.002 C -4.827 5.018 -4.899
4.998 -4.949 4.948 C -4.998 4.899 -5.018 4.827 -5.003 4.759 L -4.844 4.086 C -4.881 4.042
-4.918 3.998 -4.953 3.954 L -5.644 3.978 C -5.714 3.981 -5.780 3.947 -5.819 3.889 C -5.858
3.830 -5.864 3.756 -5.835 3.692 L -5.549 3.064 C -5.577 3.014 -5.604 2.963 -5.631 2.912 L
-6.311 2.801 C -6.380 2.789 -6.438 2.743 -6.465 2.679 C -6.492 2.614 -6.483 2.540 -6.443
2.483 L -6.040 1.924 C -6.058 1.869 -6.075 1.813 -6.091 1.758 L -6.736 1.516 C -6.802
1.491 -6.849 1.435 -6.863 1.366 C -6.877 1.298 -6.854 1.227 -6.804 1.179 L -6.299 0.708 C
-6.305 0.651 -6.311 0.594 -6.315 0.537 L -6.903 0.173 C -6.963 0.137 -7.000 0.072 -7.000
0.001 C -7.000 -0.069 -6.963 -0.134 -6.903 -0.171 L -6.315 -0.534 C -6.311 -0.592 -6.305
-0.649 -6.299 -0.706 L -6.804 -1.177 C -6.855 -1.225 -6.878 -1.296 -6.864 -1.364 C -6.850
-1.433 -6.802 -1.490 -6.736 -1.514 L -6.091 -1.756 C -6.075 -1.812 -6.058 -1.867 -6.040
-1.922 L -6.443 -2.481 C -6.484 -2.538 -6.493 -2.613 -6.466 -2.677 C -6.439 -2.742 -6.380
-2.789 -6.311 -2.799 L -5.630 -2.910 C -5.604 -2.961 -5.577 -3.012 -5.548 -3.062 L -5.835
-3.690 C -5.864 -3.754 -5.858 -3.828 -5.819 -3.887 C -5.780 -3.945 -5.713 -3.979 -5.643
-3.976 L -4.953 -3.952 C -4.917 -3.997 -4.881 -4.041 -4.844 -4.085 L -5.002 -4.758 C
-5.018 -4.826 -4.998 -4.898 -4.948 -4.947 C -4.898 -4.997 -4.827 -5.017 -4.759 -5.001 L
-4.086 -4.842 C -4.042 -4.880 -3.998 -4.916 -3.953 -4.951 L -3.977 -5.642 C -3.980 -5.712
-3.947 -5.779 -3.888 -5.818 C -3.830 -5.857 -3.755 -5.863 -3.692 -5.833 L -3.064 -5.547 C
-3.013 -5.575 -2.962 -5.602 -2.911 -5.629 L -2.800 -6.309 C -2.788 -6.378 -2.742 -6.436
-2.678 -6.463 C -2.613 -6.490 -2.539 -6.482 -2.482 -6.442 L -1.923 -6.039 C -1.868 -6.057
-1.812 -6.074 -1.756 -6.090 L -1.515 -6.735 C -1.491 -6.801 -1.434 -6.850 -1.365 -6.864 C
-1.296 -6.877 -1.225 -6.854 -1.178 -6.802 L -0.706 -6.298 C -0.650 -6.304 -0.592 -6.309
-0.535 -6.315 L -0.171 -6.902 C -0.134 -6.962 -0.069 -6.998 0.001 -6.998 C 0.070 -6.998
0.135 -6.962 0.172 -6.902 L 0.536 -6.315 C 0.593 -6.309 0.651 -6.304 0.707 -6.298 L 1.178
-6.802 C 1.226 -6.853 1.297 -6.876 1.365 -6.862 C 1.434 -6.848 1.490 -6.800 1.515 -6.735 L
1.757 -6.090 C 1.813 -6.074 1.868 -6.057 1.923 -6.039 L 2.483 -6.442 C 2.539 -6.483 2.614
-6.492 2.679 -6.465 C 2.744 -6.438 2.790 -6.379 2.800 -6.309 L 2.911 -5.629 C 2.963 -5.602
3.014 -5.575 3.064 -5.547 L 3.692 -5.833 C 3.756 -5.862 3.830 -5.855 3.888 -5.817 C 3.946
-5.778 3.980 -5.712 3.978 -5.642 L 3.954 -4.951 C 3.999 -4.916 4.043 -4.880 4.086 -4.842 L
4.759 -5.001 C 4.827 -5.017 4.898 -4.996 4.948 -4.947 C 4.997 -4.897 5.018 -4.826 5.002
-4.758 L 4.844 -4.085 C 4.880 -4.041 4.917 -3.997 4.952 -3.952 L 5.643 -3.976 C 5.714
-3.979 5.781 -3.946 5.820 -3.887 C 5.859 -3.829 5.865 -3.754 5.835 -3.690 L 5.549 -3.063 C
5.577 -3.012 5.604 -2.961 5.631 -2.910 L 6.311 -2.799 C 6.380 -2.787 6.438 -2.741 6.465
-2.677 C 6.492 -2.612 6.483 -2.538 6.443 -2.481 L 6.040 -1.922 L 6.091 -1.756 L 6.736
-1.514 C 6.802 -1.490 6.851 -1.433 6.864 -1.364 C 6.878 -1.296 6.855 -1.225 6.804 -1.177 L
6.299 -0.706 C 6.305 -0.649 6.311 -0.592 6.315 -0.534 L 6.903 -0.171 C 6.963 -0.134 7.000
-0.069 7.000 0.001 C 7.000 0.072 6.963 0.137 6.903 0.173 Z M 2.971 -4.701 C 2.747 -4.652
2.605 -4.431 2.653 -4.207 C 2.701 -3.983 2.921 -3.840 3.145 -3.886 C 3.293 -3.916 3.413
-4.022 3.460 -4.165 C 3.507 -4.308 3.473 -4.465 3.372 -4.576 C 3.270 -4.687 3.117 -4.735
2.970 -4.701 Z M 2.771 -3.351 C 2.673 -3.330 2.570 -3.348 2.486 -3.403 C 2.401 -3.458
2.342 -3.544 2.321 -3.642 L 2.113 -4.616 C 1.469 -4.908 0.755 -5.070 0.002 -5.070 C -0.743
-5.072 -1.479 -4.909 -2.154 -4.596 L -2.362 -3.622 C -2.383 -3.524 -2.442 -3.438 -2.527
-3.383 C -2.611 -3.329 -2.714 -3.310 -2.812 -3.331 L -3.671 -3.516 C -3.831 -3.351 -3.979
-3.176 -4.116 -2.992 L 0.066 -2.992 C 0.113 -2.992 0.145 -2.983 0.145 -2.940 L 0.145
-1.461 C 0.145 -1.418 0.113 -1.410 0.066 -1.410 L -1.157 -1.410 L -1.157 -0.472 L 0.165
-0.472 C 0.286 -0.472 0.811 -0.506 0.979 -1.177 C 1.031 -1.383 1.146 -2.055 1.225 -2.269 C
1.304 -2.510 1.624 -2.992 1.965 -2.992 L 4.049 -2.992 C 4.074 -2.991 4.099 -2.989 4.124
-2.984 C 3.980 -3.180 3.822 -3.366 3.651 -3.540 Z M -3.012 -4.681 C -3.158 -4.715 -3.312
-4.667 -3.413 -4.556 C -3.515 -4.445 -3.549 -4.288 -3.502 -4.145 C -3.455 -4.002 -3.334
-3.895 -3.187 -3.866 C -2.964 -3.822 -2.746 -3.965 -2.699 -4.188 C -2.651 -4.410 -2.790
-4.629 -3.012 -4.681 Z M -4.598 1.752 C -4.533 1.615 -4.546 1.453 -4.635 1.330 C -4.723
1.207 -4.871 1.141 -5.021 1.158 C -5.172 1.176 -5.301 1.274 -5.359 1.414 C -5.444 1.622
-5.348 1.861 -5.142 1.952 C -4.937 2.043 -4.695 1.954 -4.598 1.752 Z M -5.085 0.596 L
-4.190 0.994 C -4.098 1.035 -4.026 1.111 -3.990 1.204 C -3.954 1.298 -3.957 1.403 -3.997
1.495 L -4.182 1.912 L -3.456 1.912 L -3.456 -1.356 L -4.919 -1.356 C -5.100 -0.722 -5.156
-0.059 -5.085 0.597 Z M -1.157 0.913 L -1.157 1.876 L 0.570 1.876 C 0.659 1.876 1.199
1.773 1.199 1.369 C 1.199 1.033 0.785 0.913 0.444 0.913 Z M 5.118 0.046 C 5.118 -0.081
5.114 -0.208 5.104 -0.334 L 4.579 -0.334 C 4.527 -0.334 4.505 -0.368 4.505 -0.420 L 4.505
-0.661 C 4.505 -1.228 4.185 -1.352 3.905 -1.383 C 3.638 -1.413 3.342 -1.271 3.305 -1.108 C
3.148 -0.222 2.885 -0.032 2.471 0.294 C 2.985 0.621 3.520 1.103 3.520 1.747 C 3.520 2.444
3.043 2.883 2.717 3.098 C 2.261 3.399 1.755 3.459 1.619 3.459 L -3.810 3.459 C -3.060
4.298 -2.054 4.866 -0.948 5.075 L -0.308 4.404 C -0.238 4.331 -0.143 4.289 -0.042 4.286 C
0.058 4.284 0.155 4.322 0.228 4.391 L 0.944 5.076 C 2.421 4.799 3.702 3.887 4.446 2.582 L
3.956 1.475 C 3.872 1.283 3.958 1.059 4.149 0.974 L 5.092 0.555 C 5.109 0.387 5.117 0.218
5.117 0.046 Z M -0.307 5.646 C -0.200 5.748 -0.046 5.786 0.097 5.744 C 0.240 5.702 0.349
5.587 0.384 5.443 C 0.419 5.299 0.374 5.146 0.267 5.044 C 0.099 4.899 -0.153 4.911 -0.306
5.072 C -0.460 5.232 -0.460 5.485 -0.307 5.646 Z M 4.557 1.732 C 4.602 1.832 4.685 1.911
4.787 1.951 C 4.890 1.991 5.005 1.988 5.105 1.943 C 5.259 1.875 5.357 1.721 5.353 1.552 C
5.350 1.384 5.244 1.234 5.087 1.174 C 4.930 1.113 4.752 1.153 4.636 1.275 C 4.520 1.397
4.488 1.577 4.557 1.731 Z};}%
\sbox{\osvlogo}{\includegraphics[height=\logoh]{osv}}%
\sbox{\depsdevlogo}{\tikz[line cap=round]{%
  \draw[branddepsdevdark, line width=2.2pt] (-0.07,-0.07) -- (-0.21,-0.21);
  \draw[branddepsdev, line width=1.6pt] (0,0) circle[radius=0.17];
  \draw[branddepsdev, line width=1.3pt] (0.01,0.02) circle[radius=0.06];
  \draw[branddepsdev, line width=1.6pt] (-0.04,-0.04) -- (-0.21,-0.21);}}%
\newsavebox{\termicon}%
\newsavebox{\cpuicon}\newsavebox{\charticon}%
\sbox{\termicon}{\tikz{%
  \filldraw[draw=otgray!90!black, fill=otgray!85!black, rounded corners=1pt, line width=0.4pt]
    (0,0) rectangle (0.5,0.36);
  \fill[otgray!40] (0,0.30) rectangle (0.5,0.36);
  \node[text=white, font=\ttfamily\tiny\bfseries, inner sep=0pt, anchor=west] at (0.05,0.15) {>\_};}}%
\sbox{\cpuicon}{\tikz[scale=0.17]{%
  \foreach \i in {1,...,5}{
    \pgfmathsetmacro{\p}{-1.1 + 2.2*(\i-0.5)/5}
    \draw[otgray!70, line width=0.5pt] (\p,1.1) -- (\p,1.4);
    \draw[otgray!70, line width=0.5pt] (\p,-1.1) -- (\p,-1.4);
    \draw[otgray!70, line width=0.5pt] (1.1,\p) -- (1.4,\p);
    \draw[otgray!70, line width=0.5pt] (-1.1,\p) -- (-1.4,\p);}
  \filldraw[draw=otpurple!80!black, fill=otpurple!15, rounded corners=1pt, line width=0.45pt]
    (-1.1,-1.1) rectangle (1.1,1.1);
  \filldraw[draw=otpurple!80!black, fill=otpurple!35, line width=0.4pt] (-0.5,-0.5) rectangle (0.5,0.5);}}%
\sbox{\charticon}{\tikz[line width=0.4pt]{%
  \draw[otgray!80] (0,0) -- (0.5,0);
  \fill[otblue!70] (0.05,0) rectangle (0.14,0.16);
  \fill[otteal!80] (0.19,0) rectangle (0.28,0.30);
  \fill[otorange!90] (0.33,0) rectangle (0.42,0.22);}}%
\newsavebox{\pkgicon}\newsavebox{\calicon}\newsavebox{\sliicon}%
\sbox{\pkgicon}{\tikz[scale=0.12, line width=0.35pt]{%
  \filldraw[draw=otteal!75!black, fill=otteal!16] (0,0) rectangle (1.8,1.8);
  \filldraw[draw=otteal!75!black, fill=otteal!28] (0,1.8) -- (0.6,2.4) -- (2.4,2.4) -- (1.8,1.8) -- cycle;
  \filldraw[draw=otteal!75!black, fill=otteal!22] (1.8,0) -- (2.4,0.6) -- (2.4,2.4) -- (1.8,1.8) -- cycle;}}%
\sbox{\calicon}{\tikz[line width=0.35pt]{%
  \filldraw[draw=otorange!80!black, fill=white, rounded corners=0.5pt] (0,0) rectangle (0.28,0.26);
  \fill[otorange!80!black] (0,0.19) rectangle (0.28,0.26);
  \foreach \x in {0.06,0.14,0.22}{ \foreach \y in {0.05,0.12}{ \fill[otgray!70] (\x-0.02,\y) rectangle (\x+0.02,\y+0.035); } }}}%
\sbox{\sliicon}{\tikz[line width=0.4pt]{%
  \foreach \y/\x in {0.04/0.18, 0.13/0.08, 0.22/0.14}{
    \draw[otgray!80] (0,\y) -- (0.28,\y);
    \filldraw[draw=otblue!75!black, fill=otblue!35] (\x,\y) circle[radius=0.035]; }}}%
\newsavebox{\histicon}%
\sbox{\histicon}{\tikz[line width=0.55pt]{%
  \draw[otblue!75!black, -{Stealth[length=1.1mm, width=1.3mm]}] (-60:0.2) arc[start angle=-60, end angle=200, radius=0.2];
  \draw[otblue!75!black, line width=0.6pt, line cap=round] (0,0) -- (0,0.12) (0,0) -- (0.08,-0.04);
  \fill[otblue!75!black] (0,0) circle[radius=0.025];}}%
\newsavebox{\deptreeicon}%
\sbox{\deptreeicon}{\tikz[line width=0.45pt]{%
  \draw[otgray!80] (0,0.1) -- (-0.13,-0.06) (0,0.1) -- (0.13,-0.06);
  \filldraw[draw=otblue!75!black, fill=otblue!35, rounded corners=0.5pt] (-0.06,0.07) rectangle (0.06,0.17);
  \filldraw[draw=otblue!75!black, fill=white, rounded corners=0.5pt] (-0.19,-0.12) rectangle (-0.07,-0.02);
  \filldraw[draw=otblue!75!black, fill=white, rounded corners=0.5pt] (0.07,-0.12) rectangle (0.19,-0.02);
  \filldraw[draw=otorange!85!black, fill=white, line width=0.45pt] (0.19,0.13) circle[radius=0.075];
  \draw[otorange!85!black, line width=0.4pt, line cap=round] (0.19,0.13) -- (0.19,0.18) (0.19,0.13) -- (0.225,0.13);}}%
\newsavebox{\cacheicon}\newsavebox{\indexicon}%
\sbox{\cacheicon}{\tikz[line width=0.45pt]{%
  \filldraw[draw=otorange!85!black, fill=otorange!55, rounded corners=0.8pt] (0,0) rectangle (0.42,0.12);
  \fill[otorange!85!black] (0.34,0.06) circle[radius=0.02];
  \filldraw[draw=otorange!85!black, fill=white, rounded corners=0.8pt] (0,0.17) rectangle (0.42,0.29);
  \foreach \x in {0.06,0.13,0.2,0.27}{ \fill[otorange!85!black] (\x,0.21) rectangle (\x+0.04,0.25); }}}%
\sbox{\indexicon}{\tikz[line width=0.4pt]{%
  \filldraw[draw=otteal!75!black, fill=white] (0,0) rectangle (0.36,0.28);
  \fill[otteal!75!black] (0,0.21) rectangle (0.36,0.28);
  \foreach \y in {0.07,0.14}{ \draw[otteal!60] (0,\y) -- (0.36,\y); }
  \draw[otteal!60] (0.12,0) -- (0.12,0.21);
  \filldraw[draw=otgray!90!black, fill=white, line width=0.55pt] (0.33,0.08) circle[radius=0.075];
  \draw[otgray!90!black, line width=0.9pt, line cap=round] (0.385,0.025) -- (0.44,-0.03);}}%
\newsavebox{\dashicon}\newsavebox{\ideicon}\newsavebox{\githubicon}%
\sbox{\dashicon}{\tikz[line width=0.4pt]{%
  \filldraw[draw=otblue!70!black, fill=white, rounded corners=0.8pt] (0,0) rectangle (0.5,0.36);
  \fill[otblue!70!black] (0,0.29) rectangle (0.5,0.36);
  \foreach \x in {0.04,0.09,0.14}{ \fill[white] (\x,0.325) circle[radius=0.012]; }
  \fill[otblue!70] (0.08,0.04) rectangle (0.15,0.14);
  \fill[otteal!80] (0.2,0.04) rectangle (0.27,0.23);
  \fill[otorange!90] (0.32,0.04) rectangle (0.39,0.18);}}%
\sbox{\ideicon}{\tikz[line width=0.4pt]{%
  \filldraw[draw=otpurple!80!black, fill=white, rounded corners=0.8pt] (0,0) rectangle (0.5,0.36);
  \fill[otpurple!80!black] (0,0) rectangle (0.1,0.36);
  \node[text=otpurple!80!black, font=\ttfamily\tiny\bfseries, inner sep=0pt] at (0.3,0.17) {</>};}}%
\sbox{\githubicon}{\scalebox{1.75}{\tikz{%
  \fill[brandgithub] svg {%
    M 3.6 7.111 C 1.611 7.111 0 5.499 0 3.511 C 0 1.92 1.031 0.571 2.462 0.095 C
    2.642 0.062 2.708 0.173 2.708 0.269 C 2.708 0.354 2.705 0.581 2.703 0.881 C
    1.702 0.663 1.49 1.364 1.49 1.364 C 1.327 1.779 1.09 1.89 1.09 1.89 C
    0.764 2.113 1.115 2.109 1.115 2.109 C 1.477 2.084 1.667 1.738 1.667 1.738
    C 1.988 1.187 2.509 1.346 2.715 1.439 C 2.747 1.671 2.84 1.83 2.943 1.92 C
    2.144 2.01 1.303 2.32 1.303 3.699 C 1.303 4.092 1.443 4.413 1.674 4.665 C
    1.633 4.756 1.512 5.122 1.705 5.618 C 1.705 5.618 2.007 5.714 2.695
    5.249 C 2.983 5.329 3.289 5.369 3.595 5.37 C 3.901 5.369 4.207 5.329
    4.495 5.249 C 5.179 5.714 5.481 5.618 5.481 5.618 C 5.674 5.122 5.553
    4.756 5.517 4.665 C 5.746 4.413 5.886 4.092 5.886 3.699 C 5.886 2.316 5.044
    2.012 4.243 1.923 C 4.369 1.815 4.486 1.594 4.486 1.257 C 4.486 0.775 4.482
    0.388 4.482 0.271 C 4.482 0.177 4.545 0.064 4.729 0.1 C 6.17 0.572 7.2 1.922
    7.2 3.511 C 7.2 5.499 5.588 7.111 3.6 7.111%
  };}}}%


